Convergence to Nash Equilibrium and No-regret Guarantee in (Markov) Potential Games

In this work, we study potential games and Markov potential games under stochastic cost and bandit feedback. We propose a variant of the Frank-Wolfe algorithm with sufficient exploration and recursive gradient estimation, which provably converges to the Nash equilibrium while attaining sublinear regret for each individual player. Our algorithm simultaneously achieves a Nash regret and a regret bound of $O(T^{4/5})$ for potential games, which matches the best available result, without using additional projection steps. Through carefully balancing the reuse of past samples and exploration of new samples, we then extend the results to Markov potential games and improve the best available Nash regret from $O(T^{5/6})$ to $O(T^{4/5})$. Moreover, our algorithm requires no knowledge of the game, such as the distribution mismatch coefficient, which provides more flexibility in its practical implementation. Experimental results corroborate our theoretical findings and underscore the practical effectiveness of our method.

==> congestion.tex <==
\section{Congestion game}

As a classic example of the potential game, we apply our algorithm to the special case of a congestion game. The main challenge inherent to congestion games lies in the potentially exponentially large strategy space.

In a congestion game, we have a set of resources $\mathcal{E}$ and $n$ players choosing strategy $a_i$, which is a combination of different facilities, i.e. $a_i \in A_i \subseteq 2^{[d]}$, $d = |\mathcal{E}|$. Each player can also employ a randomized (mixed) strategy $\pi_i$, and play an action $a_i$ sampled from $\pi_i$. For every resource $e \in \mathcal{E}$, we use $N_e(a)$ to denote the number of players who have chosen that particular resource. Each player receive a cost $c_i(a) = \sum_{e \in a_i} \bar{c}_i(e, N_e(a))$, where $\bar{c}_i(e,N_e(a))$ is a cost function related to resource $e$, and depends on $N_e(a)$. In the stochastic setting, each player may only have access to a sampled cost $\bar{C}_i(e, N_e(a))$ from a distribution of mean $\bar{c}_i(e, N_e(a))$. Without loss of generality, we assume $\bar{C}_i(e, N_e(a)) \in [0,1]$ for all strategy $a$ and resource $e$. We note $C_i(a) = \sum_{e \in a_i} \bar{C}_i(e, N_e(a))$ and we slightly abuse the notation and let $c_i(\pi) = \EE_{a \sim \pi} [c_i(a)]$.

In the repeated game setting, throughout a time horizon $T$, all players take a strategy $a^t$ based on their mixed strategy $\pi^t$ at each time step $t \in [T]$. Subsequently, they receive some feedback on their chosen strategies. Then they use this cost information to update their strategy. In general, there are two types of partial information feedback in this repeated game setting. 

\begin{itemize}
    %\item \textbf{Full-information feedback}: After taking the action $a^t \sim \pi^t$, player $i$ observes $\bar{C}_i(e, N_e((a, a_{-i}^t)))$ for all $a \in \mathcal{A}_i$, $e \in \mathcal{E}$. 
    \item \textbf{Semi-bandit feedback}: After taking the actions $a^t \sim \pi^t$, player $i$ observes $\bar{C}_i(e, N_e(a_i^t, a_{-i}^t))$.
    \item \textbf{Bandit feedback}: After taking the actions $a^t \sim \pi^t$, player $i$ observes $C_i(a^t) = \sum_{e \in a_i^t}\bar{C}_i(e, N_e(a^t))$.
\end{itemize}


\subsection{Algorithm}

\paragraph{Decomposing the strategy space}
To address the challenge posed by the exponentially large strategy space, we leverage the implicit description of the strategy space with on Carathéodory Decomposition. This offers significant improvement in both the sample and time complexities of Algorithm \ref{alg}, allowing the regret and the computation complexity to be only logarithmic in $m$. We remark that the same idea has been previously applied in congestion game \cite{panageas23} and combinatorial optimization \cite{korte2011combinatorial}.

Fix a player $i$ and given a action $a_i$, we can describe it as $x_{a_i} \triangleq\left\{x \in\{0,1\}^d: x_e=1 \text { iff } e \in a_i\right\}$ \cite{kleer2021computation}. Consider the set $\hat{A}_i = \left\{x_{\pi_i} \in [0,1]^d \right\}$ and the polytope $\mathcal{X}_i:=\operatorname{conv}\left(\mathcal{A}_i\right)$ denoting the convex hull of $\mathcal{A}_i$. This polytope $\mathcal{A}_i$ can also be described alternatively as $\mathcal{X}_i := \left\{x \in [0,1]^d : A_i \cdot x \leq b_i\right\}$, where $A_i \in \mathbb{R}^{r \times d}$ and $b_i \in \mathbb{R}^r$. Consequently, $\mathcal{A}_{i}$ can be implicitly characterized as the extreme points of a set $\mathcal{X}_{i} := \left\{x \in [0,1]^d : A_i \cdot x \leq b_i\right\}$, which can be represented using $\mathcal{O}(\mathrm{rd})$ fractional numbers.

Formally, this is known as the Carathéodory Decomposition \cite{caratheodory1911variabilitatsbereich,steinitz1913bedingt}
\begin{thm}[Carathéodory Decomposition]
For any point $x \in \mathcal{X}_i$ there exists a probability distribution $\pi_x \in \Delta\left(\mathcal{A}_i\right)$ with support at most $d+1$ actions $a_i$ in $\mathcal{A}_i$ such that for all facilities $f \in \mathcal{F}$,
$$
x_e=\sum_{a_i: e \in a_i} \mathbb{P}_{\pi_x}\left[a_i \text{ is selected } \right] \,.
$$
Such a distribution (it may not be unique) $\pi_x$ is called a Carathéodory decomposition of $x$.
\end{thm}

To effectively use the Carathéodory decomposition, \citet{panageas23} defines the following potential function, for which our Algorithm \ref{alg} can optimize efficiently. 
\begin{defn}[\cite{panageas23}]
\label{def:potential_x}
Let the fractional potential function $\psi$ be
\[\psi(x) = \inf_{A\pi = x} \Phi(\pi) = \sum_{e \in \mathcal{E}} \sum_{\mathcal{S} \subset[n]} \prod_{j \in \mathcal{S}} x_{j, e} \prod_{k \notin \mathcal{S}}\left(1-x_{k, e}\right) \sum_{i=0}^{|\mathcal{S}|} u(e,i) \,.\]
Then, for any randomized (mixed) strategy $\pi = (\pi_i, \pi_{-i})$, $\pi_i^\prime$, $c_i(\pi_i, \pi_{-i}) - c_i(\pi_i^\prime,  \pi_{-i}) = \psi(x_i, x_{-i}) - \psi(x_i^\prime,  x_{-i})$, where $\pi_i$, $\pi_{-i}$ are the Carathéodory decomposition of $x_i, x_{-i}$
\end{defn}

\paragraph{Cost estimator}
To apply Algorithm \ref{alg} in the congestion game, we would need a one-sample unbiased gradient estimator (line 4 of Algorithm \ref{alg}) to build the recursive gradient estimator. 

Under semi-bandit feedback, we can leverage importance sampling to estimate the cost for each facility.  
\begin{align}\label{eq:semi_bandit_cost_est}
    \text{Semi-bandit feedback: } \quad \hat{C}^t_{i,e} = \frac{\bar{C}^t_i(e, N_e(a^t)) \mathbb{I}\{e \in a_i^t\}}{x_e^t}\,, \forall e \in \mathcal{E} \,.
\end{align}

Under bandit feedback, we use an estimator that is similar to the one used in adversarial linear bandit. 
\begin{align}\label{eq:bandit_cost_est}
\text{Bandit feedback: } \quad   \hat{C}_t = C^t_i(a^t) (\Sigma^t)^{-1} a_i^t \,, \quad \Sigma^t = \EE_{\pi_i^t} [a_i a_i^\top]\,.
\end{align}
One can show that both of these estimates are unbiased, and have bounded norms. 
%{\color{blue}TODO: explain the algorithm}

Algorithm \ref{alg:congestion} gives an overview of stochastic Frank-Wolfe with exploration that can be applied to the congestion game. It has the same structure as Algorithm \ref{alg}, but with the Frank-Wolfe update step performed on $\mathcal{X}_i$ to overcome the exponentially large action space. 
\begin{algorithm}
\KwInput{Parameters $\eta_t$, $\rho_t$, $\mu$.}
\For{$t = 1, \ldots, T$}{
    $y_i^{t} = (1 - m\mu)x_i^{t} + m\mu s_i$, $s = 1/(kn) \sum^n_{\ell=1} a^\ell$, and $\{a^\ell\}$ is a collection of strategies that covers every resource\;
    Play $a_i^t \sim \tilde{\pi}_i^t$, where $ \tilde{\pi}_i^t$ is a Carathéodory decomposition of $y_i^{t}$ and receive cost $C^t_i$\;
    Estimate cost with Equation \ref{eq:bandit_cost_est} (Bandit feedback) or Equation \ref{eq:semi_bandit_cost_est} (Semi-bandit feedback)\;
    Update $d^t_i = (1-\rho_t)d^{t-1}_i + \rho_t \hat{C}_i^t$\;
    Update $\hat{x}_i^{t+1} = \argmin_{x_i} \langle x_i, d^t_i \rangle$\;
    Update $x_i^{t+1} = (1-\eta_t)x_i^t + \eta_t \hat{x}_i^{t+1}$\;
}
\caption{Stochastic Frank-Wolfe with exploration for congestion game}\label{alg:congestion}
\end{algorithm}

To derive a theoretical guarantee of Algorithm \ref{alg:congestion}, we maintain the following assumption. 
\begin{asmp}\label{asmp:congestion}
    We assume that each pure strategy $a_i \in \mathcal{A}_i$, $i \in [n]$, is consists of $k$ resources. 
\end{asmp}




\subsection{Results for congestion game}
\begin{restatable}[Nash regret (bandit feedback)]{thm}{nashregretbandit}
\label{thm:nash_congestion_bandit}
With $\eta = \frac{2}{t^{4/5}} $, $\mu = \frac{1}{n^{3/8} d^{d^{17/16} } T^{1/5}}$ and $\rho_t = \frac{4\mu^{1/3}d^{1/6}}{t^{8/15}}$, we have
\begin{align*}
        \EE\left[\text{Nash-Regret}(T) \right]
        = O \left(n^{29/8} d^{3/2} T^{1-\beta} + (n^{29/8}+n^{17/8}\sqrt{k})d^{3/2} T^{4/5} \right)  \,.
        %= O \left( \left(( n^{4.5} d^{2} + n^{1.5}\sqrt{dC} \right) T^{4/5} + n^3 d^{1.5} T^{1/5}\right)  \,,
    \end{align*}
    %$C = \max\left\{C_1,\frac{2n^4 d + n^2k^4}{\lambda^2} + 6n^3 d^{1.5} \right\}$, $C_1$ is a constant and 
    %where $\lambda$ be the smallest nonzero eigenvalue of $\EE[a a^\top]$ and $a$ is a uniform exploration action. 
\end{restatable}
\begin{rem}
    When $T \geq O \left(\frac{n^{18.125}d^{7.5}}{\epsilon^5}\right)$, there exists a $t \in \{1, \ldots, T\}$, such that $\pi^t$ is an $\epsilon$-equilibrium.
\end{rem}
\begin{rem}
    Using Markov inequality, it is immediate that Theorem \ref{thm:nash_regret} also holds with high probability. 
\end{rem}

\begin{restatable}[Individual regret (bandit feedback)]{thm}{individualregretbandit}\label{thm:individual_congestion_bandit}
With $\eta_t = \frac{2}{t^{4/5}} $, $\mu = \frac{1}{n^{3/8} d^{17/16} T^{1/5}}$ and $\rho_t = \frac{4\mu^{1/3}d^{1/6}}{t^{8/15}}$, we have
\begin{align*}
    \sum^T_{t=1} c_i(\pi_i^t, \pi_{-i}^t) -  \min_{\pi_i^\ast}\sum^T_{t=1}c_i(\pi_i^\ast, \pi_{-i}^t) = O\left( \left(n^{2} d^{3/2} + \left(n^{21/8}+\sqrt{k}\right)d^{3/2}\right)T^{4/5}\right) \,.
    %= \ & O \left(n^3d^2 T^{4/5} + \frac{\left(n^2d + nk^2 \sqrt{d}\right) T^{4/5}}{\lambda}\right)\,,
    %=  O \left(n^2d T^{4/5} + D T^{4/5}\right) \,,
\end{align*}
%where $D =\max \left\{D_1, 4n^2d^{1.5} + 8n^3 d^{2} + 4\sqrt{dC}\right\}$, $C = \max\left\{C_1,\frac{2n^4 d + n^2k^4}{\lambda^2} + 6n^3 d^{1.5} \right\}$, $C_1, D_1$ are constants, and 
where $\lambda$ be the smallest nonzero eigenvalue of $\EE[a a^\top]$ and $a$ is a uniform exploration action. 
\end{restatable}

Compared to the previous results of $O(n^{1.5} d^{2.5} T^{4/5})$(Nash regret) and $O(d^2 n^2 T^{4/5})$ (individual player regret) under the more informative semi-bandit feedback setting, our result obtains the same order of $O(T^{4/5})$ regrets under the stricter setting of full-bandit feedback. %In the semi-bandit feedback setting, we improve the result to $O(n^{4.5} d^2 T^{7/9})$ for Nash regret and $O(n^3 d^2 T^{7/9})$ in Theorem \ref{thm:nash_congestion_semi} and Theorem \ref{thm:individual_congestion_semi}. 


==> congestion_analysis.tex <==
\section{Analysis for congestion game}
\subsection{Proof to Theorem \ref{thm:nash_congestion_bandit}}
%\nashregretbandit*
\begin{proof}
We start by decomposing the regret as,
\begin{align*}
        \mathrm{Nash-regret}(T)
        = \ & \sum^T_{t=1} \max_i \left(c_i\left(\pi_i^t, \pi_{-i}^t\right) - \min_{\hat{\pi}_i} c_i\left(\hat{\pi}_i, \pi_{-i}^t\right)\right) \\
        \leq \ & \sum^n_{i=1} \sum^T_{t=1} \max_{\hat{\pi}_i} \left(c_i\left(\pi_i^t, \pi_{-i}^t\right) -  c_i\left(\hat{\pi}_i, \pi_{-i}^t\right)\right) \\
        = \ & \sum^n_{i=1} \sum^T_{t=1} \max_{\hat{x}_i} \left(\psi\left(x_i^t, x_{-i}^t\right) -  \psi\left(\hat{x}_i, x_{-i}^t\right)\right) + \sum^n_{i=1}\sum^T_{t=1} \left( \psi(y_i^t, x_{-i}^t) - \psi(x_i^t,x_{-i}^t) \right) \\
        \leq \ & \sum^n
        _{i=1} \sum^T_{t=1} \max_{\hat{x}_i} \left(\psi\left(x_i^t, x_{-i}^t\right) -  \psi\left(\hat{x}_i, x_{-i}^t\right)\right) + 2n^2 d^2 \mu T\,,
    \end{align*}
    where the last inequality is by Lemma \ref{lem:explore}.

    Define $G(x^t) = \max_x (x^t - x)^\top \nabla_{x} \psi(x^t)$.

    %{\color{blue}TODO: }
    By the smoothness of $\psi$, we have
    \begin{align*}
        \psi(x^{t+1}) 
        \leq \ & \psi(x^t) + (x^{t+1} - x^t)^\top \nabla_{x} \psi(x_i) + n^2 \sqrt{d} \|x^{t+1} - x^t\|_2^2 \\
        \leq \ & \psi(x^t) + \eta_t (\hat{x}^{t+1} - x^t)^\top \nabla_{x} \psi(x^t) + \eta_t^2 n^2 \sqrt{d} \|\hat{x}^{t+1} - x^t\|_2^2 \\
        = \ & \psi(x^t) + \eta_t(\hat{x}^{t+1} - x^t)^\top d^t + \eta_t(\hat{x}^{t+1} - x^t)^\top \left(\nabla_{x} \psi(x^t)  - d^t\right) + \eta_t^2 n^2 \sqrt{d} \|\hat{x}^{t+1} - x^t\|_2^2\\
        \leq \ & \psi(x^t) + \eta_t(\hat{x}^{t+1} - x^t)^\top d^t + \eta_t \sqrt{nd} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \eta_t^2 n^2 d^{1.5}\,.
    \end{align*}
    where the second inequality is by update rule, the third equality is by Cauchy-Schwarz inequality, and that $x \in \mathcal{X}_i$ is a binary vector with dimension $d$.

    Let $\Tilde{x}^{t+1} = \argmin_{x} \langle x, \nabla_{x} \psi(x^t)\rangle$.
    Then 
    \begin{align*}
        & \psi(x^{t+1}) \\
        \leq \ &  \psi(x^t) + \eta_t(\hat{x}^{t+1} - x^t)^\top d^t + \eta_t \sqrt{nd}  \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \eta_t^2 n^2 d^{1.5} \\
        \leq \ & \psi(x^t) + \eta_t(\Tilde{x}^{t+1} - x^t)^\top d^t + \eta_t \sqrt{nd} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \eta_t^2 n^2 d^{1.5} \\
        = \ &  \psi(x^t) + \eta_t(\Tilde{x}^{t+1} - x^t)^\top \nabla_{x} \psi(x^t) + \eta_t(\Tilde{x}^{t+1} - x^t)^\top \left(d^t - \nabla_{x} \psi(x^t) \right)+ \eta_t \sqrt{nd} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \eta_t^2 n^2 d^{1.5} \\
        \leq \ &  \psi(x^t) - \eta_t G(x^t) + 2\eta_t \sqrt{nd} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \eta_t^2 n^2 d^{1.5} \,,
    \end{align*}
    where the second inequality is by the update rule, and the third inequality is by the definition of $G(x_i^t)$ and Cauchy-Schwarz. 

    Rearrange the terms gives 
    \begin{align*}
        G(x^t) \leq \ & \frac{\psi(x^t) - \psi(x^{t+1})}{\eta_t} +2 \sqrt{nd} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \eta n^2 d^{1.5} \,.
    \end{align*}
    
    Summing over $T$ gives
    \begin{align*}
        \sum^{T}_{t=1} G(x^t) 
        \leq \ & \sum^{T}_{t=1}\frac{\psi(x^t) - \psi(x^{t+1})}{\eta_t} + 2\sqrt{nd} \sum^{T}_{t=1} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \sum^{T}_{t=1}\eta_t n^2 d^{1.5}  \\
        = \ & \sum^{T}_{t=1} \left(\left(\frac{\psi(x^t)}{\eta_t} - \frac{\psi(x^{t+1})}{\eta_{t+1}}\right) + \left(\frac{1}{\eta_{t+1}} - \frac{1}{\eta_{t}}\right)\psi(x^{t+1})\right) + 2\sqrt{nd} \sum^{T}_{t=1} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \sum^{T}_{t=1}\eta_t n^2 d^{1.5} \\
        \leq \ & \left(\frac{\psi(x^1)}{\eta_1} - \frac{\psi(x^{T+1})}{\eta_{T+1}}\right) + \frac{d}{\eta_T} + 2\sqrt{nd} \sum^{T}_{t=1} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 + \sum^{T}_{t=1}\eta_t n^2 d^{1.5} \\
        \leq \ & \frac{2nd}{\eta_T} + 2\sqrt{nd} \sum^{T}_{t=1} \left\|\nabla_{x} \psi(x^t)  - d^t\right\|_2 +  \sum^{T}_{t=1}\eta_t n^2 d^{1.5} \,,
    \end{align*}
    where the second inequality is because $\eta_t \geq \eta_{t+1}$. 

    Since $\psi$ is a linear function of $x^t$, by Taylor expansion we have $\psi\left(x\right) = \psi\left(x^t\right) - (x - x^t)^\top \nabla_{x}\psi\left(x^t\right) $. Therefore, we have
    \begin{align*}
        c_i\left(\pi_i^t, \pi_{-i}^t\right) - \min_{\hat{\pi}_i} c_i\left(\hat{\pi}_i, \pi_{-i}^t\right)
        = \ & \max_{\hat{x}_i} \left(\psi\left(x_i^t, x_{-i}^t\right) -  \psi\left(\hat{x}_i, x_{-i}^t\right)\right) \\
        = \ & \max_{\hat{x}_i} (x_i^t - \hat{x}_i)^\top \nabla_{x} \psi\left(x_i^t, x_{-i}^t\right) \\
        \leq \ & \max_{x} \left(x^t - x\right)^\top \nabla_{x}\psi\left(x^t\right) = G(x^t) \,.
    \end{align*}

    Thus, for a fixed $i \in [n]$, we have
    \begin{align*}
       \EE\left[ \sum^{T}_{t=1} \left(c_i\left(\pi_i^t, \pi_{-i}^t\right) - \min_{\hat{\pi}_i} c_i\left(\hat{\pi}_i, \pi_{-i}^t\right)\right) \right]
        \leq \ & \frac{2nd}{\eta_T} + 2\sqrt{nd} \sum^{T}_{t=1} \left\|\nabla_{x} \psi(x^t)  - d^t\right\| + n^2 d^{1.5} \sum^T_{t=1} \eta_t  \,.
    \end{align*}

    With $\eta_t = \frac{1}{n^{3/2}d^{3/4}t^{3\alpha/2}} $, $\rho_t = \frac{4\mu^{1/3}}{(n^{4/3}d^{1/3}+(kd)^{1/3})t^\alpha}$, $\mu \leq \frac{1}{2}$, by Lemma \ref{lem:est_diff}, we have
    \begin{align*}
        2\sqrt{nd}\sum^{T}_{t=1} \EE \left[\|\nabla_{x} \psi\left(x^t\right) - d_t \|_2 \right] \leq \ &  O \left(n^{3}d^{3/2}\mu T+ \frac{n^{3/2}d^{5/6}+\sqrt{n}k^{1/3}d^{5/6}T^{1-\alpha/2}}{\mu^{1/3}}\right)\,.
    \end{align*}
    %where $C = \max\left\{C_1,\frac{2n^4 d + n^2k^4}{\lambda^2} + 6n^3 d^{1.5} \right\}$ and $C_1$ is a constant. 

    Therefore, for a fixed $i$, taking $\mu = \frac{1}{n^{9/8}\sqrt{d}T^\beta}$, we have
    \begin{align*}
        &\EE\left[\sum^T_{t=1}\left(c_i\left(\pi_i^t, \pi_{-i}^t\right) - \min_{\hat{\pi}_i} c_i\left(\hat{\pi}_i, \pi_{-i}^t\right)\right) \right] \\
        = \ & O \left(n^{5/2}d^{7/4} T^{3\alpha/2} + n^{15/8}d\mu T+ n^{15/8}k^{1/3}dT^{1-\alpha/2 + \beta/3} + \sqrt{n} d^{3/4} T^{1-3\alpha/2}\right)\,.
    \end{align*}

    Take $\alpha = 8/15$, $\beta = 1/5$, we have
    \begin{align*}
        \EE\left[\text{Nash-Regret}(T) \right]
        = O \left( n^{7/2}d^{7/4} T^{4/5} + n^{23/8}k^{1/3}dT^{4/5} \right) \,.
    \end{align*}
    %where $C = \max\left\{C_1,\frac{2n^4 d + n^2k^4}{\lambda^2} + 6n^3 d^{1.5} \right\}$ and $C_1$ is a constant. 
    
\end{proof}
\subsection{Nash regret (semi-bandit feedback) }

\begin{thm}[Nash regret (semi-bandit feedback)]\label{thm:nash_congestion_semi}
Take $\eta = 2t^{-4/5}$, $\mu = \frac{1}{(nd)^{3/8}T^{1/5}}$, $\rho_t = \frac{4\mu^{1/3}d^{1/6}}{n^{1/3}t^{8/15}}$, we have
\begin{align*}
    \EE \left[\text{Nash-regret}(T)\right]
    = \ & O \left(n^{29/8}d^{9/8} T^{4/5}\right) \,.
    %= \ & O \left(\left(n^{1.5}\sqrt{dC} + n^{4.5}d^2 \right) T^{7/9} + n^3 d^{1.5} T^{2/9}\right)\,.
\end{align*}
   %where $C = \max\left\{C_1 ,3n^4d  + 6n^3 d^{1.5}\right\}$, and $C_1$ is a constant.
\end{thm}

\begin{proof}
    The proof is mostly the same with Theorem \ref{thm:nash_congestion_bandit}. Following the same argument, take $\eta_t =  \frac{1}{n^{3/2}d^{3/4}t^{3\alpha/2}} $, $\rho_t = \frac{4\mu^{1/3}}{n^{4/3}d^{1/3}t^\alpha}$ and $\mu = \frac{d^{1/4}}{n^{7/8}T^\beta}$, with Lemma \ref{lem:est_diff_semibandits}, for a fixed $i \in [n]$, we have
    \begin{align*}
        & \EE\left[ \sum^{T}_{t=1} \left(c_i\left(\pi_i^t, \pi_{-i}^t\right) - \min_{\hat{\pi}_i} c_i\left(\hat{\pi}_i, \pi_{-i}^t\right)\right) \right] \\
        \leq \ & \frac{2nd}{\eta_T} + 2\sqrt{nd} \sum^{T}_{t=1} \left\|\nabla_{x} \psi(x^t)  - d^t\right\| + n^2 d^{1.5} \sum^T_{t=1} \eta_t  \\
        \leq \ & \frac{2nd}{\eta_T} +  O \left(n^3d^{3/2}\mu T +  \frac{  n^{11/6}d^{7/6}T^{1-\alpha/2}}{\mu^{1/3}} \right) + n^2 d^{1.5} \sum^T_{t=1} \eta_t \\
        \leq \ & O \left(n^{5/2}d^{7/4}T^{3\alpha/2} + \sqrt{n}d^{3/4}T^{1-3\alpha/2} + n^{17/8}d^{5/4} \left(T^{1-\beta} + T^{1-\alpha/2+\beta/3}\right)\right)\,.
    \end{align*}

    % \ref{lem:est_diff_semibandits}, we have
    % \begin{align*}
    %      & \EE\left[ \sum^{T}_{t=1} \left(c_i\left(\pi_i^t, \pi_{-i}^t\right) - \min_{\hat{\pi}_i} c_i\left(\hat{\pi}_i, \pi_{-i}^t\right)\right) \right] \\
    %     = \ & O \left(n^{5/2}d^{7/4} T^{3\alpha/2}  + n^{13/8} d^{9/8}T^{1-\beta}+ \sum^T_{t=1}\frac{n^{21/8}d^{9/8}}{t^{\alpha/2-\beta/3}} + n^2 d^{1.5} T^{1-3\alpha/2}\right) \,,
    % \end{align*}
    %where $C = \max\left\{C_1 ,3n^4d  + 6n^3 d^{1.5}\right\}$, and $C_1$ is a constant.
    Combining everything and take $\alpha = 8/15$, $\beta = 1/5$, we have
    \begin{align*}
        \EE \left[\text{Nash-regret}(T)\right]
        = \ & O \left(n^{7/2}d^{7/4} T^{4/5}\right) \,.
    \end{align*}
\end{proof}


\subsection{Proof to Theorem \ref{thm:individual_congestion_bandit}}
%\individualregretbandit*

\begin{proof}
{\color{blue}TODO: fix}
Denote $\pi^\ast = \argmin_\pi \sum^T_{t=1} c_i(\pi, \pi_{-i}^t)$ and $x^\ast$ be the corresponding decomposition, by the definition of the potential function, we have
\begin{align*}
    \sum^T_{t=1} c_i(\pi_i^t, \pi_{-i}^t) -  c_i(\pi_i^\ast, \pi_{-i}^t)
    = \ & \sum^T_{t=1} \psi(y_i^t, x_{-i}^t) -  \psi(x_i^\ast, x_{-i}^t) \\
    = \ & \sum^T_{t=1}\left( \psi(y_i^t, x_{-i}^t) - \psi(x_i^t, x_{-i}^t)\right) + \sum^T_{t=1}\left( \psi(x_i^t, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \right)\\
    \leq \ & 2d^2n\mu T+ \sum^T_{t=1}\left( \psi(x_i^t, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \right) \,.
\end{align*}

By the smoothness of $\psi$, we have
\begin{align*}
    & \psi(x_i^{t+1}, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \\
    = \ & \psi((x_i^t + \eta_t (\hat{x}_i^{t+1} - x_i^t), x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \\
    \leq \ & \left(\psi(x_i^{t}, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \right)+ \eta_t \langle\hat{x}_i^{t+1} - x_i^t , \nabla_{x_i} \psi(x_i^{t}, x_{-i}^t)\rangle + \eta_t^2 n^2 \sqrt{d} \|\hat{x}_i^{t+1} - x_i^t\|^2\\
    \leq \ &  \left(\psi(x_i^{t}, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \right)+ \eta_t \langle\hat{x}_i^{t+1} - x_i^t , \nabla_{x_i} \psi(x_i^{t}, x_{-i}^t)\rangle + \eta_t^2 n^2 d^{1.5} \,.
\end{align*}

For the second term, notice that
\begin{align*}
    \langle\hat{x}_i^{t+1} - x_i^t , \nabla_{x_i} \psi(x_i^{t}, x_{-i}^t)\rangle
    = \ & \langle\hat{x}_i^{t+1} - x_i^t , d^t\rangle + \langle\hat{x}_i^{t+1} - x_i^t , \nabla_{x_i} \psi(x_i^{t}, x_{-i}^t) - d^t\rangle \\
    \leq \ & \langle x_i^\ast - x_i^t , d^t\rangle + \sqrt{d} \|\nabla_{x_i} \psi(x_i^{t}, x_{-i}^t) - d^t\|_2 \\
    \leq \ &  \langle x_i^\ast - x_i^t ,\nabla_{x_i} \psi(x_i^{t}, x_{-i}^t)\rangle + \langle x_i^\ast - x_i^t , d^t - \nabla_{x_i} \psi(x_i^{t}, x_{-i}^t)\rangle  + \sqrt{d} \|\nabla_{x_i} \psi(x_i^{t}, x_{-i}^t) - d^t\|_2 \\
    \leq \ & \left( \psi(x_i^\ast, x_{-i}^t) - \psi(x_i^t, x_{-i}^t) \right) + 2\sqrt{d} \|\nabla_{x_i} \psi(x_i^{t}, x_{-i}^t) - d^t\|_2 \,,
\end{align*}
where the first inequality is by the update rule, $\hat{x}_i^{t+1} = \argmin \langle x, d^t \rangle$, and the last inequality is because $\psi$ is linear in $x_i$.

Therefore, we have
\begin{align*}
    \psi(x_i^{t+1}, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) 
    \leq \ & (1 - \eta_t) \left( \psi(x_i^\ast, x_{-i}^t) - \psi(x_i^t, x_{-i}^t) \right) + 2\eta_t \sqrt{d}\|\nabla_{x_i} \psi(x_i^{t}, x_{-i}^t) - d^t\|_2 + \eta_t^2 n^2d^{1.5} \,.
\end{align*}

By Lemma \ref{lem:est_diff} and take $\eta_t = 2/t^{3\alpha/2}$, we have
\begin{align*}
    & \EE \left[\psi(x_i^{t+1}, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \right] \\
    \leq \ & \left(1 - \frac{2}{t^{3\alpha/2}}\right) \EE\left[ \left( \psi(x_i^t, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \right)\right] + \frac{4n^2d^{1.5}}{t^{3\alpha}}
    + O \left(\frac{n^{2.5} d^{3/2}\mu}{t^{3\alpha/2}} + \frac{(n^2+\sqrt{k})d^{13/12}}{\mu^{1/3}t^{2\alpha}}\right)\,,
\end{align*}
%where $C = \max\left\{C_1,\frac{2n^4 d + n^2k^4}{\lambda^2} + 6n^3 d^{1.5} \right\}$, and $C_1$ is a constant.

Denote $a_{t+1} = \EE \left[\psi(x_i^{t+1}, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) \right] $, we have
\begin{align*}
    a_{t+1} \leq \left(1 - \frac{2}{t^{3\alpha/2}}\right)a_t +  \frac{4n^2d^{1.5}}{t^{3\alpha}}
    + O \left(\frac{n^{2.5} d^{3/2}\mu}{t^{3\alpha/2}} + \frac{(n^2+\sqrt{k})d^{13/12}}{\mu^{1/3}t^{2\alpha}}\right)\,.
\end{align*}

Take $\alpha = 8/15$, $\mu_t = \frac{1}{n^{3/8}d^{17/16}t^{1/5}}$, we have
\begin{align*}
    a_{t+1} 
    %\leq \ & \left(1 - \frac{2}{t^{4/5}}\right)a_t +  \frac{4n^2d^{1.5}}{t^{8/5}}
    %+ \frac{8n^3 d^{2}}{t} + \frac{4\sqrt{dC}}{t}\\
    \leq \ & \left(1 - \frac{2}{t^{4/5}}\right)a_t +  O\left( n^2d^{3/2} + n^{17/16} d^{7/16} + (n^{21/8}+\sqrt{k})d^{23/16}\right)\frac{1}{t} \,.
\end{align*}

We now show that $a_t \leq D t^{-1/5}$ by induction, where $D =\max \left\{a_1, O\left( n^{2} d^{3/2} + (n^{21/8}+\sqrt{k})d^{3/2}\right)\right\}$.

When $t = 1$, we have $a_1 \leq D /1 $, which is true by the definition of D. Assume $a_t \leq D t^{-1/5}$, for $t \geq 2$. Then for $t + 1$, we have
\begin{align*}
    a_{t+1} 
    %\leq \ & \left(1 - \frac{2}{t^{4/5}}\right)\frac{D}{t^{1/5}} + \left(4n^2d^{2.5} + 8n^4 d^{2.5} + 4d\max\left\{C,\frac{2n^4 d + n^2k^4}{\lambda^2} + 6n^2 d \right\}\right) \frac{1}{t}\\
    \leq \ & \left(1 - \frac{2}{t^{4/5}}\right)\frac{D}{t^{1/5}} +  \frac{D}{t} \\
    = \ & \frac{D}{t^{1/5}} - \frac{D}{t} 
    = \frac{D}{t^{1/5}} \left(\frac{1}{t^{4/5} +1}\right) = \frac{D}{t^{1/5} + t} \leq \frac{D}{t^{1/5} + 1} \leq \frac{D}{(t+1)^{1/5} } \,.
\end{align*}

Putting everything together and by Lemma \ref{lem:explore}, we have
\begin{align*}
    \sum^T_{t=1} c_i(\pi_i^t, \pi_{-i}^t) -  c_i(\pi_i^\ast, \pi_{-i}^t)
    = \ & O\left( \left(n^{2} d^{3/2} + \left(n^{21/8}+\sqrt{k}\right)d^{3/2}\right)T^{4/5}\right) \,.
    %\leq \ & 2n^2d\sum^T_{t=1}  t^{-1/5} + D\sum^T_{t=1} t^{-1/5} = O \left(n^2d T^{4/5} + D T^{4/5}\right) \,.
\end{align*}


\end{proof}
\subsection{Individual regret (semi-bandit feedback)}
{\color{blue}TODO: fix}
\begin{thm}[Individual regret (semi-bandit feedback)]\label{thm:individual_congestion_semi}
Take $\eta = 2t^{-4/5}$, $\mu = \frac{1}{(nd)^{3/8}T^{1/5}}$, $\rho_t = \frac{4\mu^{1/3}d^{1/6}}{n^{1/3}t^{8/15}}$, we have
\begin{align*}
        \sum^T_{t=1} c_i(\pi_i^t, \pi_{-i}^t) -  \min_{\pi_i^\ast}\sum^T_{t=1}c_i(\pi_i^\ast, \pi_{-i}^t)
        = n^2 d^{3/2} T^{4/5}\,.
    %= O \left(n^2d T^{2/9} + D T^{7/9}\right)\,,
    \end{align*}
    %where $D = \max\{a_1, 8n^3d^2 + 4\sqrt{dC} +  4n^2 d^{1.5}\}$, $C = \max\left\{C_1 ,3n^4d  + 6n^3 d^{1.5}\right\}$ and $C_1, D_1$ are constants. 
\end{thm}

\begin{proof}
    The proof is similar to that of Theorem \ref{thm:individual_congestion_bandit}. Therefore, let $a_t =  \psi(x_i^{t+1}, x_{-i}^t) - \psi(x_i^\ast, x_{-i}^t) $, we have
    \begin{align*}
        a_t
    \leq \ & (1 - \eta_t) a_{t-1} + 2\eta_t \sqrt{d}\|\nabla_{x_i} \psi(x_i^{t}, x_{-i}^t) - d^t\|_2 + \eta_t^2 n^2d^{1.5} \,.
    \end{align*}
    Take $\eta_t =  \frac{1}{t^{3\alpha/2}} $, $\rho_t = \frac{4\mu^{1/3}d^{1/6}}{n^{1/3}t^\alpha}$, $\mu = \frac{1}{(nd)^{3/8}T^\beta}$ and by Lemma \ref{lem:est_diff_semibandits}, we have
    \begin{align*}
        a_t
    \leq \ & \left(1 - \frac{2}{t^{3\alpha/2}}\right) a_{t-1} + O \left( \frac{n^{5/2} d^{3/2} \mu}{t^{3\alpha/2}}+\frac{n^2d}{\mu^{1/3}t^{2\alpha}} \right) +  \frac{4n^2d^{1.5}}{t^{3\alpha}} \\
    \leq \ & \left(1 - \frac{2}{t^{3\alpha/2}}\right) a_{t-1} + O \left( \frac{n^{17/16} d^{9/8} }{t^{3\alpha/2+ \beta}}+\frac{n^{17/16} d^{9/8} }{\mu^{1/3}t^{2\alpha - \beta/3}} \right) +  \frac{4n^2d^{1.5}}{t^{3\alpha }} \,.
    \end{align*}
    %where $C = \max\left\{C_1 ,3n^4d  + 6n^3 d^{1.5}\right\}$, and $C_1$ is a constant. 

    Take $\beta = 1/5$ and $\alpha = 8/15$, we have
    \begin{align*}
        a_t \leq \ & \left(1 - \frac{2}{t^{7/9}}\right) a_{t-1} + O \left(n^2 d^{1.5}\right) \frac{1}{t} \,.
    \end{align*}
    Define $D = \max\{a_1, O \left(n^2 d^{1.5}\right)\}$, and $a_t \leq Dt^{-1/5}$ by induction proof from Theorem \ref{thm:individual_congestion_bandit}. 

    
    Therefore, we have
    \begin{align*}
        \sum^T_{t=1} c_i(\pi_i^t, \pi_{-i}^t) -  \min_{\pi_i^\ast}\sum^T_{t=1}c_i(\pi_i^\ast, \pi_{-i}^t)
    = O \left(n^2 d^{3/2} T^{4/5}\right)\,.
    \end{align*}
    %where $D = \max\{D_1,8n^2d^{2.5} + 8d\sqrt{\max\left\{C_1 ,3n^4d  + 6n^2 d^{1.5}\right\}} +  8n^2 d^{1.5}\}$, and $D_1$ is a constant. 
    
\end{proof}

\subsection{Auxiliary Lemmas}
\begin{lem}\label{lem:congestion_smooth}
The potential function $\psi(\cdot)$ is smooth. More precisely,
$$
\left\|\nabla \psi(x)-\nabla \psi\left(x^{\prime}\right)\right\|_2 \leq 2 n^2  \sqrt{d} \cdot\left\|x-x^{\prime}\right\|_2
$$
for all $x, x^{\prime}$.
\end{lem}
\begin{lem}\label{lem:explore}
        For $y_i = (1 - d \mu)x_i + d \mu s$, where $s = 1/(kd) \sum^d_{\ell=1} a^\ell$, and $\{a^\ell\}$ is a collection of strategies that covers every resource, we have $\psi(y_i, x_{-i}) - \psi(x_i,x_{-i}) \leq 2 d^2 n  \mu$.
    \end{lem}
    \begin{proof}
    This is proved in Lemma 14 of \cite{panageas23}. Let $\mathcal{E}$ denote the set of facilities. 
    By 
        \begin{align*}
        \psi(y_i, x_{-i}) - \psi(x_i,x_{-i})
        = \ & \sum_{e \in \mathcal{E}} \sum_{\mathcal{S} \subset[n], i \in \mathcal{S}}\left(x_{i e}-(1-d \mu) x_{i e}-d \mu s\right) \prod_{j \in \mathcal{S}, j \neq i} x_{j e} \prod_{j \notin \mathcal{S}}\left(1-x_{j e}\right) \sum_{l=0}^{|\mathcal{S}|} c_e(l) \\
        + \ & \sum_{e \in \mathcal{E}} \sum_{\mathcal{S} \subset[n], i \notin \mathcal{S}}\left(-x_{i e}+(1-d \mu) x_{i e}+ d \mu s\right) \prod_{j \in \mathcal{S}} x_{j e} \prod_{j \notin \mathcal{S}, j \neq i}\left(1-x_{j e}\right) \sum_{l=0}^{|\mathcal{S}|} c_e(l) \\
        \leq \ &  \sum_{e \in \mathcal{E}}n \left(x_{i e}-(1-d \mu) x_{i e}-d \mu s\right)  \underbrace{\sum_{\mathcal{S} \subset[n], i \in \mathcal{S}} \prod_{j \in \mathcal{S}, j \neq i} x_{j e} \prod_{j \notin \mathcal{S}}\left(1-x_{j e}\right)}_{=1} \\
        + \ & \sum_{e \in \mathcal{E}} n\left(-x_{i e}+(1-d \mu) x_{i e} +d \mu s\right)  \underbrace{\sum_{\mathcal{S} \subset[n], i \notin \mathcal{S}} \prod_{j \in \mathcal{S}} x_{j e} \prod_{j \notin \mathcal{S}, j \neq i}\left(1-x_{j e}\right)}_{=1} \\
        = \ & 2 d^2 n \mu \,.
\end{align*}
    \end{proof}

\begin{lem}\label{lem:grad}
    $ \EE [\hat{C}_i^t]  = \nabla_{x_i} \psi(x^t) $.
\end{lem}
\begin{proof}
By the definition of $\hat{C}^t$, we have
\begin{align*}
    \EE [\hat{C}^t] 
    = \ & \EE \left[C_i^t(a^t) (\Sigma^t)^{-1} a_i^t\right] 
    = \ \EE \left[(\Sigma^t)^{-1} a_i^t (a_i^t)^\top C_i^t(a^t)\right]
    = \ (\Sigma^t)^{-1} \Sigma^t c_i^t = \EE [C_i^t]\,,
\end{align*}
The second inequality is by Theorem 5.1 of \cite{panageas23}.
{\color{blue} Let's assume everything is invertible for now. In the general case, we need to use the pseudoinverse.}
   % The first statement is proved in the proof of Theorem 6 of \cite{combes2015combinatorial}. The second statement is proved in \cite{cuilearning}.
\end{proof}


\begin{lem}\label{lem:grad_norm}[Theorem 6 of \cite{combes2015combinatorial}]
    Let $\EE_t$ denote the conditional expectation on the history up to time $t$, then $\EE_t \left[\left\|\hat{C}^t_i\right\|_2\right] \leq \frac{k^{3/2}}{\mu \lambda}$, and $\EE_t \left[\left\|\hat{C}^t_i\right\|_2^2\right] \leq \frac{kd}{(1-\mu)}$, where $\lambda$ be the smallest nonzero eigenvalue of $\EE[a a^\top]$ and $a$ is a uniform exploration action.
\end{lem}
\begin{proof}
    % \begin{align*}
    %     \left\|\hat{C}^t_i\right\|_2
    %     = \ & \left\|C^t_i(a^t) (\Sigma^t)^{-1} a_i^t \right\|_2 \\
    %     \leq \ & k \left\|C^t_i(a^t) (\Sigma^t)^{-1}  \right\|_2 \\
    %     \leq \ &  k \left\|C^t_i(a^t) \right\|_2 \sqrt{\lambda_{\max} ((\Sigma^t)^{-1}(\Sigma^t)^{-1})} \\
    %     \leq \ & k^{3/2} \lambda_{\max} ((\Sigma^t)^{-1}) \,,
    % \end{align*}
    % where the first and third inequality is by the assumption that each strategy consists of $k$ facilities. 

    % Note that $\lambda_{\max} ((\Sigma^t)^{-1}) = \frac{1}{\lambda_{\min} ((\Sigma^t))}$, and 
    % \begin{align*}
    %     \lambda_{\min} ((\Sigma^t))
    %     = \ & \min_{\|x\|_2 = 1, x \in \text{span}(\hat{\mathcal{A}}_i)} x^\top \Sigma^t x \\
    %     = \ & \EE \left[x^\top a^t (a^t)^\top x \right] \geq \mu \EE \left[ \left(a^\top x\right)^2\right] \,,
    % \end{align*}
    % where $a$ is a uniform exploration action and the last inequality is by the mixing (exploration step). 

    % Let $\lambda$ be the smallest nonzero eigenvalue of $\EE[a a^\top]$, then $\lambda_{\min} ((\Sigma^t)) \leq \mu \lambda$. 

    %By Lemma 4 of 
\end{proof}

\begin{lem}[Theorem 5.1 of \cite{panageas23}] \label{lem:grad_norm_semi}

\begin{enumerate}
    \item $\EE[\hat{C}_i^t] = \nabla_{x_i} \psi(x_i^t, x_{-i}^t)$.
    \item  $\EE\left[\|\hat{C}_i^t\|^2\right] \leq \frac{d}{\mu}$.
\end{enumerate}
    
\end{lem}

\begin{lem}[Gradient estimation error (bandit feedback)]\label{lem:est_diff_bandit}
With $\eta_t =  \frac{1}{n^{3/2}d^{3/4}t^{3\alpha/2}} $, $\rho_t = \frac{4\mu^{1/3}}{(n^{4/3}d^{1/3}+(kd)^{1/3})t^\alpha}$, $\mu \leq \frac{1}{2}$, we have
    \begin{align*}
     \EE \left[\|\nabla_{x} \psi\left(x^t\right) - d_t \|_2 \right] \leq \ O \left(n^{5/2}d\mu + \frac{n^{4/3}d^{1/3}+(kd)^{1/3}}{\mu^{1/3}t^{\alpha/2}}\right)\,.
\end{align*}
%where $C = \max\left\{C_1,\frac{2n^4 d + n^2k^4}{\lambda^2} + 6n^3 d^{1.5} \right\}$, and $C_1$ is a constant.
\end{lem}
\begin{proof}
    We first decompose $\|\nabla_{x} \psi\left(x^t\right) - d^t\|_2^2$ as 
    \begin{align*}
        \|\nabla_{x} \psi\left(x^t\right) - d^t \|_2
        \leq \ &  \|\nabla_{x} \psi\left(x^t\right) - \nabla_{y} \psi\left(y^t\right) \|_2 +\|\nabla_{x} \psi\left(y^t\right) - d^t\|_2 \\
        \leq \ & 2n^2 \sqrt{d} \|x^t - y^t\|_2^2 + \|\nabla_{x} \psi\left(y^t\right) - d^t\|_2 \\
        \leq \ & 2n^{5/2} d \mu + \|\nabla_{x} \psi\left(y^t\right)-  d^t\|_2\,,
    \end{align*}
    where the second inequality is the smoothness of $\psi$ and the third inequality is by the update rules of our algorithm. 
\begin{align*}
    & \left\||\nabla_{x} \psi\left(y^t\right) - d^t \right\|_2^2 \\
    = \ & \left\|\nabla_{x} \psi\left(y^t\right) - (1-\rho_t) d^{t-1} - \rho_t\hat{C}^t\right\|_2^2 \\
    = \ & \left\|\rho_t\left(\nabla_{x} \psi\left(y^t\right) - \hat{C}^t\right) + (1-\rho_t) \left( \nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right) + (1-\rho_t) \left( \nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\right)\right\|_2^2 \\
    \leq \ & \rho_t^2 \left\|\nabla_{x} \psi\left(y^t\right) - \hat{C}^t\right\|_2^2 + (1-\rho_t)^2 \left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 + (1-\rho_t)^2\left\| \nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\right\|_2^2 \\
    & \ + 2 \rho_t(1-\rho_t) \left\langle \nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1} ,\nabla_{x} \psi\left(y^t\right) - \hat{C}^t\right\rangle \\
    & \ + 2\rho_t(1 - \rho_t) \left\langle \nabla_{x} \psi\left(y^t\right) - \hat{C}^t , \nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right) \right\rangle\\
    & \ + 2 (1-\rho_t)^2 \left\langle \nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1},  \nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\right\rangle \,.
\end{align*}
Taking expectations on both sides and recalling that the one-sample gradient estimate is unbiased, we have
\begin{align*}
    \EE\left[\left\||\nabla_{x} \psi\left(y^t\right) - d^t \right\|_2^2\right] 
    \leq \ & (1-\rho_t)^2 \EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \hat{C}^t\right\|^2_2\right] \\
    & \ + (1-\rho_t)^2 \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\right\|_2^2 \right] \\
    & \ + 2 (1-\rho_t)^2 \EE \left[\left\langle \nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1},  \nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\right\rangle \right] \,.
\end{align*}

Using $2\langle a, b\rangle \leq \beta_t \|a\|_2^2 + \|b\|_2^2 / \beta_t$, for $\beta_t > 0$, we have
\begin{align*}
    &  \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - d_t \right\|_2^2\right]  \\
    \leq \ & (1-\rho_t)^2 \EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \hat{C}^t\right\|_2^2\right] \\
    & \ + (1-\rho_t)^2 \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\right\|_2^2 \right]  + \beta_t(1-\rho_t)^2 \EE \left[\| \nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1} \|_2^2\right] \\
    & \ + (1-\rho_t)^2/\beta_t\EE \left[\| \nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\|_2^2\right]\\
    \leq \ & (1-\rho_t)(1+\beta_t) \EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \hat{C}^t\right\|_2^2\right] \\
    & \ + (1-\rho_t)(1 + 1/\beta_t) \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right)\right\|_2^2 \right] \,.
\end{align*}

Set $\beta_t = \rho_t / 2$, we have
\begin{align*}
    & \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - d_t \right\|_2^2\right] \\
    \leq \ & (1-\rho_t/2)\EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \hat{C}^t\right\|_2^2\right] \\
    & \ + (1 + 2/\rho_t) \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - \nabla_{x} \psi\left(y^{t-1}\right) \right\|_2^2 \right] \\
    \leq \ & (1-\rho_t/2) \EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\left(2n^4 d + \frac{kd}{(1-\mu)}\right) + (1 + 2/\rho_t) 2n^2 \sqrt{d}\EE\left[\left\| y^t - y^{t-1}\right\|_2^2 \right] \\
    %\leq \ &  (1-\rho_t/2)\EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \frac{\rho_t^2 (2n^4 d + k^4)}{\mu^2 \lambda^2} \\
    %& \ + 2m^2 \sqrt{n}(1 + 2/\rho_t) \EE\left[\left\| (1 - n \mu_{t})x_i^{t} - (1 - n \mu_{t-1})x_i^{t-1} + s (n \mu_{t} - n \mu_{t-1})\right\|_2^2 \right]  \\
    \leq \ & (1-\rho_t/2)\EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \frac{\rho_t^2 (2n^4 d + kd)}{1-\mu} + 2n^2 \sqrt{d}(1 + 2/\rho_t)  (1 - d \mu)\EE\left[\left\|x^{t} - x^{t-1} \right\|_2^2 \right] \\
    %\leq \ & (1-\rho_t/2) \EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \frac{\rho_t^2 (2m^4 n + k^2)}{\mu_t \lambda} + 2m^2 \sqrt{n}\eta^2(1 + 2/\rho_t)\EE\left[\left\|\hat{x}_i^{t} - x_i^{t-1} \right\|_2^2 \right] \,,
\end{align*}
where the second inequality is by the smoothness and Lemma \ref{lem:grad_norm}, and the third inequality is because of the update rules.


By the update rules, we have $\left\|x^{t} - x^{t-1} \right\|_2^2  \leq  \eta_t^2 \left\|  \hat{x}^t - x^{t-1} \right\|_2^2 \leq \eta^2 n d $.

Therefore, we have
\begin{align*}
    \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - d_t \right\|_2^2\right] 
    \leq \ & (1-\rho_t/2)\EE \left[\left\|\nabla_{x} \psi\left(y^{t-1}\right) - d^{t-1}\right\|_2^2 \right] + \frac{\rho_t^2 (2n^4 d + kd)}{1-\mu} + \frac{6\eta_t^2 n^3 d^{1.5}}{\rho_t}\,.
\end{align*}

Define $a_t =  \EE\left[\left\|\nabla_{x} \psi\left(y^t\right) - d_t  \right\|_2^2 \right] $, and take $\mu \leq 1/2$, $\eta_t =  \frac{1}{n^{3/2}d^{3/4}t^{3\alpha/2}} $ we have
\begin{align*}
    a_t 
    \leq \ & \left(1- \frac{\rho_t}{2}\right) a_{t-1} +\frac{\rho_t^2 (2n^4 d + kd)}{\mu}  + \frac{6}{\rho_t t^{3\alpha}}   \,.
\end{align*}
%{\color{blue}TODO:}
Take $\rho_t = \frac{4\mu^{1/3}}{(n^{4/3}d^{1/3}+(kd)^{1/3})t^\alpha}$. We want to show $a_t = \frac{C}{(t + 1)^{\alpha} }$, $C = \max\left\{a_1 \mu_1 2^{\alpha} ,\frac{n^{8/3}d^{2/3}+(kd)^{2/3}}{\mu^{2/3}} \right\}$. The base case clearly holds due to our choice of $C_1$. 
%{\color{blue}TODO:}
Assume the $a_{\ell-1} \leq \frac{C}{k^{\alpha}}$, then when $\mu \leq 1/\sqrt{d}$, we have
\begin{align*}
    a_\ell
     \leq \ & \left(1 - \frac{2\mu^{1/3}}{(n^{4/3}d^{1/3}+(kd)^{1/3}) \ell^\alpha}\right) \frac{C}{\ell^\alpha}  + O\left(\frac{n^{4/3} + (kd)^{1/3} d^{4/3}}{\mu^{1/3}  \ell^{2\alpha}}\right) \\
     = \ & O \left( \left(1 - \frac{2}{\ell^\alpha}\right) \frac{(n^{4/3}d^{1/3}+(kd)^{1/3}}{\mu^{1/3} \ell^\alpha} + \frac{n^{4/3}d^{1/3}+(kd)^{1/3}}{\mu^{1/3} \ell^{2\alpha}} \right)\\
     \leq \ &  O \left(C\left(\frac{\ell^\alpha - 1}{\ell^{2\alpha}}\right)\right) \\
     \leq \ & O\left(\left(\frac{C}{\ell^{\alpha}+ 1}\right)\right)  \leq  O \left(\left(\frac{C}{(\ell+1)^{\alpha}}\right) \right) \,.
\end{align*}

Therefore,
\begin{align*}
     \EE \left[\|\nabla_{x} \psi\left(y^t\right) - d_t \|_2 \right] \leq \frac{\sqrt{C
     }}{(t+1)^{\alpha/2}} \leq \ & O \left(\frac{n^{4/3}d^{1/3}+(kd)^{1/3}}{\mu^{1/3}t^{\alpha/2}}\right) \,.
\end{align*}
\end{proof}


\begin{lem}\label{lem:grad_bandit}
The one-sample gradient estimate is unbiased, that is
    $ \EE [\hat{C}_i^t] = \nabla_{x_i} \psi(x^t) $.
\end{lem}
\begin{proof}
{\color{blue}TODO: this is a bit messay.}
Let $\Usf(a)$ denote the cost matrix corresponding to action $a$. 
By the definition of $\hat{C}^t$, we have
\begin{align*}
    \EE [\hat{C}^t] 
    = \ & \EE \left[\tilde{C}^t (\Sigma^t)^{-1} a_i^t\right] 
    = \ \EE \left[(\Sigma^t)^{-1} a_i^t (a_i^t)^\top U^t(a^t)\right]
    = \ (\Sigma^t)^{-1} \Sigma^t \Usf(a) = \EE [U^t(a^t)]\,,
\end{align*}
The second equality is by Theorem 5.1 of \cite{panageas23}.
{\color{blue} Let's assume everything is invertible for now. In the general case, we need to use the pseudoinverse.}
   % The first statement is proved in the proof of Theorem 6 of \cite{combes2015combinatorial}. The second statement is proved in \cite{cuilearning}.
\end{proof}

\begin{lem}[Gradient estimation error (semi-bandit feedback)]\label{lem:est_diff_semibandits}
Take $\eta_t =  \frac{1}{n^{3/2}d^{3/4}t^{3\alpha/2}} $, $\rho_t = \frac{4\mu^{1/3}}{n^{4/3}d^{1/3}t^\alpha}$, we have
    \begin{align*}
     \EE \left[\|\nabla_x \psi(x^t) - d_t \|_2 \right] \leq O \left( n^{5/2} d \mu+\frac{n^{4/3}d^{2/3}}{\mu^{1/3}(t+1)^{\alpha/2}}  \right)\,,
\end{align*}
%where $C = \max\left\{C_1 ,3n^4d  + 6n^3 d^{1.5}\right\}$, and $C_1$ is a constant.
\end{lem}
\begin{proof}
    We first decompose $\|\nabla_x \psi(x^t) - d^t\|_2^2$ as 
    \begin{align*}
        \|\nabla_x \psi(x^t) - d^t \|_2
        \leq \ &  \|\nabla_x \psi(x^t) - \nabla_x \psi(y^t) \|_2 +\|\nabla_x \psi(y^t) - d^t\|_2 \\
        \leq \ & 2n^2 \sqrt{d} \|x^t - y^t\|_2 + \|\nabla_x \psi(y^t) - d^t\|_2 \\
        \leq \ & 2n^{5/2} d \mu + \|\nabla_x \psi(y^t)-  d^t\|_2\,,
    \end{align*}
    where the second inequality is the smoothness of $\psi$ and the third inequality is by the update rules of our algorithm. 
\begin{align*}
    & \left\||\nabla_x \psi(y^t) - d^t \right\|_2^2 \\
    = \ & \left\|\nabla_x \psi(y^t) - (1-\rho_t) d^{t-1} - \rho_t\hat{C}^t\right\|_2^2 \\
    = \ & \left\|\rho_t\left(\nabla_x \psi(y^t) - \hat{C}^t\right) + (1-\rho_t) \left(\nabla_x \psi(y^{t-1})- d^{t-1}\right) + (1-\rho_t) \left( \nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\right)\right\|_2^2 \\
    \leq \ & \rho_t^2 \left\|\nabla_x \psi(y^t) - \hat{C}^t\right\|_2^2 + (1-\rho_t)^2 \left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 + (1-\rho_t)^2\left\| \nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\right\|_2^2 \\
    & \ + 2 \rho_t(1-\rho_t) \left\langle\nabla_x \psi(y^{t-1})- d^{t-1} ,\nabla_x \psi(y^t) - \hat{C}^t\right\rangle + 2\rho_t(1 - \rho_t) \left\langle \nabla_x \psi(y^t) - \hat{C}^t , \nabla_x \psi(y^t) -\nabla_x \psi(y^{t-1})\right\rangle\\
    & \ + 2 (1-\rho_t)^2 \left\langle\nabla_x \psi(y^{t-1})- d^{t-1},  \nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\right\rangle \,.
\end{align*}
Taking expectations on both sides and recalling that the one-sample gradient estimate is unbiased, we have
\begin{align*}
    \EE\left[\left\||\nabla_x \psi(y^t) - d^t \right\|_2^2\right] 
    \leq \ & (1-\rho_t)^2 \EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_x \psi(y^t) - \hat{C}^t\right\|^2_2\right] \\
    & \ + (1-\rho_t)^2 \EE\left[\left\|\nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\right\|_2^2 \right] \\
    & \ + 2 (1-\rho_t)^2 \EE \left[\left\langle\nabla_x \psi(y^{t-1})- d^{t-1},  \nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\right\rangle \right] \,.
\end{align*}

Using $2\langle a, b\rangle \leq \beta_t \|a\|_2^2 + \|b\|_2^2 / \beta_t$, for $\beta_t > 0$, we have
\begin{align*}
    \EE\left[\left\|\nabla_x \psi(y^t) - d_t \right\|_2^2\right]  
    \leq \ & (1-\rho_t)^2 \EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_x \psi(y^t) - \hat{C}^t\right\|_2^2\right] \\
    & \ + (1-\rho_t)^2 \EE\left[\left\|\nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\right\|_2^2 \right]  + \beta_t(1-\rho_t)^2 \EE \left[\|\nabla_x \psi(y^{t-1})- d^{t-1} \|_2^2\right] \\
    & \ + (1-\rho_t)^2/\beta_t\EE \left[\| \nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\|_2^2\right]\\
    \leq \ & (1-\rho_t)(1+\beta_t) \EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_x \psi(y^t) - \hat{C}^t\right\|_2^2\right] \\
    & \ + (1-\rho_t)(1 + 1/\beta_t) \EE\left[\left\|\nabla_x \psi(y^t) - \nabla_x \psi(y^{t-1})\right\|_2^2 \right] \,.
\end{align*}

Set $\beta_t = \rho_t / 2$, we have
\begin{align*}
    & \EE\left[\left\|\nabla_x \psi(y^t) - d_t \right\|_2^2\right] \\
    \leq \ & (1-\rho_t/2)\EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\EE\left[\left\|\nabla_x \psi(y^t) - \hat{C}^t\right\|_2^2\right] \\
    & \ + (1 + 2/\rho_t) \EE\left[\left\|\nabla_x \psi(y^t) -\nabla_x \psi(y^{t-1})\right\|_2^2 \right] \\
    \leq \ & (1-\rho_t/2) \EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \rho_t^2\left(2n^4 d + \frac{nd}{\mu }\right) + (1 + 2/\rho_t) 2n^2 \sqrt{d}\EE\left[\left\| y^t - y^{t-1}\right\|_2^2 \right] \\
    \leq \ &  (1-\rho_t/2)\EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \frac{3\rho_t^2 n^4 d }{\mu} + 2n^2 \sqrt{d}(1 + 2/\rho_t)  (1 - d \mu)\EE\left[\left\|x^{t} - x^{t-1} \right\|_2^2 \right]  \,,
    %\leq \ & (1-\rho_t/2) \EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \frac{\rho_t^2 (2m^4 n + k^2)}{\mu_t \lambda} + 2m^2 \sqrt{n}\eta^2(1 + 2/\rho_t)\EE\left[\left\|\hat{x}_i^{t} - x_i^{t-1} \right\|_2^2 \right] \,,
\end{align*}
where the second inequality is by the smoothness and Lemma \ref{lem:grad_norm_semi}, the third inequality is because of the update rules.


By the update rules, we have $\left\|x^{t} - x^{t-1} \right\|_2^2  \leq  \eta_t^2 \left\|  \hat{x}^t - x^{t-1} \right\|_2^2 \leq \eta_t^2 nd $.

Therefore, we have
\begin{align*}
    \EE\left[\left\|\nabla_x \psi(y^t) - d_t \right\|_2^2\right] 
    \leq \ & (1-\rho_t/2)\EE \left[\left\|\nabla_x \psi(y^{t-1}) - d^{t-1}\right\|_2^2 \right] + \frac{3\rho_t^2 n^4 d }{\mu} + \frac{6n^3 d^{1.5} \eta_t^2}{\rho_t}\,.
\end{align*}

Define $a_t =  \EE\left[\left\|\nabla_x \psi(y^t) - d_t  \right\|_2^2 \right] $ and take $\eta_t =  \frac{1}{n^{3/2}d^{3/4}t^{3\alpha/2}} $, we have
\begin{align*}
    a_t 
    \leq \ & \left(1- \frac{\rho_t}{2}\right) a_{t-1} + \frac{3\rho_t^2 n^4 d }{\mu} + \frac{6}{\rho_t t^{3\alpha}}\,.
\end{align*}

Take $\rho_t = \frac{4\mu^{1/3}}{n^{4/3}d^{1/3}t^\alpha}$. We want to show $a_t = \frac{C}{(t + 1)^{\alpha} } $, $C = \max\left\{a_1 \mu 2^{\alpha} ,\frac{d^{2/3}n^{8/3}}{\mu^{2/3}}\right\}$. We show this by induction. 
%{\color{blue} todo: use $(1-\rho)$ to cancel $\mu$.}

The base case clearly holds due to our choice of $C$. 

Assume the $a_{\ell-1} \leq \frac{C}{k^{\alpha}}$, when $\mu \leq \frac{n}{\sqrt{d}}$,  
\begin{align*}
    a_\ell
     \leq \ & \left(1 - \frac{2\mu^{1/3}}{n^{4/3}d^{1/3}t^\alpha}\right) \frac{C}{\ell^\alpha} + O \left(\frac{d^{1/3}n^{4/3}}{\mu^{1/3}\ell^{2\alpha}}\right) \\
     \leq \ &  O\left( \left(1 - \frac{2}{\ell^\alpha}\right) \frac{d^{1/3}n^{4/3}}{\mu^{1/3}\ell^\alpha} + \frac{d^{1/3}n^{4/3}}{\mu^{1/3}\ell^{2\alpha}} \right)\\
     \leq \ & O \left(C \left(\frac{\ell^\alpha - 1}{\ell^{2\alpha}}\right) \right)\\
     \leq \ & O \left(\left(\frac{C}{\ell^{\alpha}+ 1}\right) \right) \leq O \left( \left(\frac{C}{(\ell+1)^{\alpha}}\right) \right) \,.
\end{align*}

Therefore 
\begin{align*}
     \EE \left[\|\nabla_x \psi(y^t) - d_t \|_2 \right] \leq O \left( \frac{n^{4/3}d^{2/3}}{\mu^{1/3}(t+1)^{\alpha/2}} \right)\,.
\end{align*}
%where $C = \max\left\{C_1 ,3n^4d  + 6n^3 d^{1.5}\right\}$, and $C_1$ is a constant. Combining everything yields the claimed result. 
\end{proof}

